Regularized Gradient Clipping Provably Trains Wide and Deep Neural Networks

We present and analyze a novel regularized form of the gradient clipping algorithm, proving that it converges to global minima of the loss surface of deep neural networks under the squared loss, provided that the layers are of sufficient width. The algorithm presented here, dubbed $\delta-$GClip, introduces a modification to gradient clipping that leads to a first-of-its-kind example of a step size scheduling for gradient descent that provably minimizes training losses of deep neural nets. We also present empirical evidence that our theoretically founded $\delta-$GClip algorithm is competitive with the state-of-the-art deep learning heuristics on various neural architectures including modern transformer based architectures. The modification we do to standard gradient clipping is designed to leverage the PL* condition, a variant of the Polyak-Lojasiewicz inequality which was recently proven to be true for sufficiently wide neural networks at any depth within a neighbourhood of the initialization.

==> Notation.tex <==

\section{Some Notation}\label{sec:note} 

\note{ 
 
The following come from the ``physics'' package except the inner-product~\\ ~\\
$\ip{\va}{\vb}, \abs{c}, \norm{\vd}, \pdv{L}{\vw}, \pdv[2]{L}{\vw}, \dv{W}{t}, \dd{x}, \rank (\mM),\tr(\mA),\Tr (\mB), \var{W}$
~\\ ~\\ 
$\relu$ is our definition
~\\ 
We have also defined the following calligraphic letters, 
$\cF, \cR, \cN, \cE, \cL, \cD$
~\\
}

\begin{center} 
\hl{This is the default highlight!}
\om{This is our customized highlight!}
\end{center} 

\note{ Everything below comes from the TMLR format \\
- which comes from this book, \url{https://github.com/goodfeli/dlbook_notation/}}

\vspace{0.5cm} 
\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\sA$ & A set\\
$\R$ & The set of real numbers \\
$\{0, 1\}$ & The set containing 0 and 1 \\
$\{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$[a, b]$ & The real interval including $a$ and $b$\\
$(a, b]$ & The real interval excluding $a$ but including $b$\\
$\sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\gG$ & A graph\\
$\parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\egroup 

~\\ ~\\
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$a$ & A scalar (integer or real)\\
$\va$ & A vector\\
$\mA$ & A matrix\\
$\tA$ & A tensor\\
$\mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\mI$ & Identity matrix with dimensionality implied by context\\
$\ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\ra$ & A scalar random variable\\
$\rva$ & A vector-valued random variable\\
$\rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$P(\ra)$ & A probability distribution over a discrete variable\\
$p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$ f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$ f \circ g $ & Composition of the functions $f$ and $g$ \\
$f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\log x$ & Natural logarithm of $x$ \\
$\sigma(x)$ & Logistic sigmoid, $\frac{1} {1 + \exp(-x)}$ \\
$\zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\norm{\vx}_p $ & $L^p$ norm of $\vx$ \\
$\norm{\vx}$ & $L^2$ norm of $\vx$ \\
$x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
$\argmax_{\rvx \in \R^n} f$\\  
$\argmin_{\rvx \in \R^n} f$\\
$\reg, \rect,\softmax,\sigmoid,\softplus,\Var,\standarderror$\\
\end{tabular}
\egroup


